Legibot: Generating Legible Motions for Service Robots Using Cost-Based Local Planners

With the increasing presence of social robots in various environments and applications, there is an increasing need for these robots to exhibit socially-compliant behaviors. Legible motion, characterized by the ability of a robot to clearly and quickly convey intentions and goals to the individuals in its vicinity, through its motion, holds significant importance in this context. This will improve the overall user experience and acceptance of robots in human environments. In this paper, we introduce a novel approach to incorporate legibility into local motion planning for mobile robots. This can enable robots to generate legible motions in real-time and dynamic environments. To demonstrate the effectiveness of our proposed methodology, we also provide a robotic stack designed for deploying legibility-aware motion planning in a social robot, by integrating perception and localization components.

==> sections/dynamic_legibility_vamsi.tex <==
\section{Dynamic Legibility}

\begin{itemize}
    \item
    RQ1: How can legible motions be designed and implemented in HRC systems to enhance the transparency and understand robot actions and intentions?
%    \item
%    RQ2: What methods and technologies can be employed to enable the robot to take the user's perspective, and how does this enhance the efficiency and naturalness of collaborative interactions?
%    \item
%    RQ3: How can intention prediction in HRC be improved, and what are the key factors that influence the accuracy and speed of predicting user intentions?
\end{itemize}

Three assumptions for our problem:
\begin{itemize}
    \item
    We are developing a handover task between a robot and a human.
    \item
    The robot will track the human's head pose and gaze direction to compute the legibility of its motion.
    \item
    The generation of legible motions is done in real-time, and the robot should be able to generate legible motions for different scenarios.
\end{itemize}


Trajectory synthesis within dynamic environment:

\subsection{Background: Legibility}

\begin{equation}
    \mathbf{L}(\xi) = P(G^* |\xi_{S \rightarrow Q}) =
    \frac{\exp (-C(\xi_{S \rightarrow Q})) \int \exp( -C(\xi_{Q \rightarrow G}))}
         {\int \exp (-C(\xi_{S \rightarrow G}))}
\end{equation}

\subsection{Projection of the trajectory for a given observer}
Replace $C(\xi)$ with $T(C(\xi))$ where $T$ is the projection function from the observer's frame.

\subsection{Challenges}

\begin{itemize}
    \item \textbf{Moving Observer:} when the observer position moves from point $O_A$ to $O_B$, the robot's motion should adapt.
    should we re-calculate \ref{eq:legibility} from scratch? or can we use the previous calculation?\\
    \textit{Answer:} Now we should consider $T$ as a function of time, say $T^t$:

    \item \textbf{Prediction:} when we generate trajectory for time $t_0+dt$ in the future we need to have a prediction of the observer's position at that time.\\
    \textit{Answer:} It can be simply trajectory extrapolation, or we can also predict the intention of the user and use that to predict the observer's position.
    The prediction can be represented as a probability distribution (e.g. a Gaussian distribution) over the observer's position.
    Which means, the projected cost of $C(\xi_{Q \rightarrow G})$ will be a distribution over the cost ...
\end{itemize}

\subsection{Scenario:}
Here, we explain the scenario that we are working on ...



==> sections/extra.tex <==
\section{Extra Points and Comments}


* Note that the ``shortcut heuristic'' used in traditional planners, such as DWA, is not applicable here,
since finding a shortcut even though might reduce other costs of the plan, it can increase the legibility cost.


\vspace{0.3cm}
\hl{Extra:}
In fact, optimizing the legibility function directly is not always possible [REF].
This is because that $\Delta \mathbf{L}(\xi) = 0$ or $\mathbf{L}(\xi) = 1$ might not have a solution in the finite space.
For this reason, we might need to add some constraints to the equation to make it solvable.
In the original work, Dragana et al. [X] this is done by adding a regularizer that discourage increasing the path length.
$L(\xi) = legibility(\xi) - \lambda C(\xi)$
where $C(\xi)$ is the path length, and $\lambda$ is a constant.
%    Also, Dragan and Srinivasa [X], introduce a trust region constraint on the optimization
%     to ensure the motion does not become too surprising or unpredictable to the observer.
%    This approach in the end, turns to finding a good value for a parameter $\beta$, using a user study.
Moreover, due to the iterative nature of this approach, it can compromise the real-time performance of the system.
%    Other works [NIKOLAIDIS] a gradient ascent optimization is called N times, and the solution of the last iteration is returned.

